On commutative, operator amenable subalgebras of finite von Neumann algebras

An open question, raised independently by several authors, asks if a closed amenable subalgebra of ${\mathcal B}({\mathcal H})$ must be similar to an amenable C*-algebra; the question remains open even for singly-generated algebras. In this article we show that any closed, commutative, operator amenable subalgebra of a finite von Neumann algebra ${\mathcal M}$ is similar to a commutative C*-subalgebra of ${\mathcal M}$, with the similarity implemented by an element of ${\mathcal M}$. Our proof makes use of the algebra of measurable operators affiliated to ${\mathcal M}$.

==> acoaf_mac.tex <==


%------------------------------
\RequirePackage{amsmath,amssymb,amsfonts}
%\usepackage{theorem}
\RequirePackage{amsthm}
%\RequirePackage[normalem]{ulem}  % want to use fancy underlining for definitions?

%\usepackage{mathpazo}
\usepackage[usenames]{color}

%--------------------------------------------------
% For use in math documents as a bolt-on to Paul Taylor's macros
% Last updated 09-09-06

\NeedsTeXFormat{LaTeX2e}
% load up Paul Taylor's diagram.sty macros

%\RequirePackage[UglyObsolete]{diagrams}
% noPostScript option invoked to avoid annoying rotation of diagonal labels
\RequirePackage[PS,nohug]{diagrams}
% this should now avoid annoying label rotation


%% Arrow definitions
\newarrowmiddle{o}{\circ}{\circ}{\circ}{\circ}
%\newarrowmiddle{.}{\bullet}{\bullet}{\bullet}{\bullet}

\newarrow{Maps} |--->  % for elements (a long version of \mapsto)

\newarrow{Monic}   >--->
\newarrow{Epic}      ----{>>}
\newarrow{Strict}   --o->
\newarrow{SMonic} >-o->
\newarrow{SEpic}    --o-{>>}


\newarrow{Sub}       C--->  % subobject embedding
\newarrow{Quot}    ----{>>} % map to quotient object
\newarrow{Eq} ===== % identity map/morphism
\newarrow{Dash} {}{dash}{}{dash}>
\newarrow{Dots} ....>
\newarrow{Dbl} ===={=>} % for natural transformations and the suchlike

\newcommand{\LR}[2]{\pile{\lTo^{#1} \\ \rTo_{#2} }} % sits on top of the diagrams.sty macros
\newcommand{\RL}[2]{\pile{\rTo^{#1} \\ \lTo_{#2} }} % sits on top of the diagrams.sty macros


% ---------------------------





\numberwithin{equation}{section}

%%------------------------ Theorems etc

\newcounter{pulse}[section]
\numberwithin{pulse}{section}  % all thms, etc set from pulse


%Styles for theorems, definitions, remarks
\newcommand{\Thead}[1]{{\color{Blue}\textsf{#1}}}
%\renewcommand{\thepulse}{\textcolor{Blue}{\sf\arabic{section}.\arabic{pulse}}}
% bad hack, should hack the thmhead display rather than the counter's manifestation

%-Theorems
\theoremstyle{plain}
\newtheorem{thm}[pulse]{\Thead{Theorem}}
\newtheorem*{thmstar}{\Thead{Theorem}}
\newtheorem{prop}[pulse]{\Thead{Proposition}}
\newtheorem{lem}[pulse]{\Thead{Lemma}}
\newtheorem{cor}[pulse]{\Thead{Corollary}}
%-Definitions
\theoremstyle{definition}
\newtheorem{defn}[pulse]{\Thead{Definition}}
\newtheorem*{notn}{\Thead{Notation}}
\newtheorem{eg}[pulse]{\Thead{Example}}
%-Remarks
\theoremstyle{remark}
\newtheorem{qu}[pulse]{\Thead{Question}}
\newtheorem{rem}[pulse]{\Thead{Remark}}
\newtheorem*{remstar}{\Thead{Remark}}

% Based on a hack found in D.A. Timashev's LMS article
% Tweaked by YC to get the item numbered as (i) in the list but reffed later as 1.14(i), etc.

\newcounter{YClist}[pulse]
\def\theYClist{(\roman{YClist})}
\newenvironment{labelledlist}{
        \begin{list}{
	\rm (\roman{YClist})
	}
        {\usecounter{YClist}
        \setlength{\labelwidth}{0pt}
        \setlength{\leftmargin}{0pt}
        \setlength{\itemindent}{\labelsep}
        \let\itemsep\topsep
        \ignorespaces}
        }
        {
        \end{list}\vspace{\topsep}
        }


%% -----------------------

% journals seem to want upright roman numerals in numbered lists, we need to force this if in an italic environment

\newenvironment{YCnum}{%
\begin{enumerate}
\renewcommand{\labelenumi}{{\rm(\roman{enumi})}}
\renewcommand{\theenumi}{\rm(\roman{enumi})}
}{\end{enumerate}\ignorespacesafterend}

%%-----------

\renewcommand{\emph}[1]{{\sl #1}\/}
%\newcommand{\dt}[1]{{\it\uline{#1}}\/}  % uses ulem package
\newcommand{\dt}[1]{\textcolor{Bittersweet}{\sf#1}}

\newcommand{\wtild}[1]{\widetilde{#1}}
\newcommand{\what}[1]{\widehat{#1}}

\newcommand{\wstar}{weak$^*$}


%% \newcommand{\Alg}[1][]{{\mathcal A}_{#1}}
\newcommand{\Bdd}{{\mathcal B}}
%\newcommand{\HM}{homomorphism}
\newcommand{\wstarlim}{\hbox{$w^*$\rm-}\lim}


\newcommand{\bimod}[1]{{#1}\hbox{\sf -mod-}{#1}}
%%  \newcommand{\restr}{\operatorname{\rm restr.}}

\newcommand{\al}{\alpha}

\newcommand{\Cplx}{{\mathbb C}}
\newcommand{\Nat}{{\mathbb N}}
\newcommand{\Zahl}{{\mathbb Z}}

\newcommand{\lin}{\operatorname{lin}}
\newcommand{\Sp}{\operatorname{Sp}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\supp}{\operatorname{supp}}

\newcommand{\defeq}{\overset{\textrm{def}}{=}}
\newcommand{\st}{\,\colon\,}
\newcommand{\iso}{\cong}
\newcommand{\pair}[2]{\langle #1\,,\, #2 \rangle}
\newcommand{\Pair}[2]{\left\langle #1\,,\, #2 \right\rangle}
\newcommand{\ip}[2]{\langle #1, #2 \rangle}

\newcommand{\id}[1][]{{\sf 1}_{#1}}
\newcommand{\sid}{\mathop{\sf id}}  % generic notation for identity map
\newcommand{\fu}[1]{{#1}^{\#}}  % forced unitization

\newcommand{\clin}{\overline{\lin}}
\newcommand{\abs}[1]{\vert #1\vert}
\newcommand{\Abs}[1]{\left\vert #1\right\vert}
\newcommand{\norm}[1]{\Vert #1\Vert}
\newcommand{\Norm}[1]{\left\Vert #1\right\Vert}
\newcommand{\veps}{\varepsilon}
\newcommand{\tp}{\mathop{\otimes}}
\newcommand{\ptp}{\mathop{\widehat{\otimes}}}
\newcommand{\optp}{\mathop{\widehat{\otimes}_{\rm op}}}

%% \newcommand{\Fin}{\operatorname{Fin}}  % finite subsets of a given set

%\newcommand{\farp}{\mathop{\scriptstyle\square}} % first Arens product
%\newcommand{\sarp}{\mathop{\diamond}} % first Arens product

\newcommand{\fA}{{\mathfrak A}}
\newcommand{\fB}{{\mathfrak B}}
\newcommand{\fC}{{\mathfrak C}}

\newcommand{\sB}{{\sf B}}
\newcommand{\sE}{{\sf E}}

\newcommand{\bE}{{\mathbf E}}
\newcommand{\bF}{{\mathbf F}}
\newcommand{\bM}{{\mathbf M}}

\newcommand{\bbE}{{\mathbb E}}

\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cM}{{\mathcal M}}
% \newcommand{\cR}{{\mathcal R}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cV}{{\mathcal V}}
% \newcommand{\W}{{\mathcal W}}
\newcommand{\cZ}{{\mathcal Z}}


\newcommand{\Cst}{\operatorname{C}^*}
\newcommand{\VN}{\operatorname{VN}}
\newcommand{\spr}{\rho} % spectral radius.
\newcommand{\Gelf}{{\sf G}}
\newcommand{\lip}{\operatorname{lip}}
\newcommand{\Lip}{\operatorname{Lip}}
\newcommand{\Rad}{\operatorname{Rad}}  % Jacobson radical
\newcommand{\Lin}{{\mathcal L}}
\newcommand{\Mat}{{\mathbb M}}

\newcommand{\twomat}[4]{\left(\begin{matrix}#1 & #2 \\ #3 & #4 \end{matrix}\right)}

\newcommand{\tilcH}{\widetilde{\mathcal H}}
\newcommand{\tilcM}{\widetilde{\mathcal M}}
\newcommand{\etild}{\widetilde{e}}
\newcommand{\tilthet}{\widetilde{\theta}}
\newcommand{\tilphi}{\widetilde{\phi}}
\newcommand{\tilsB}{\widetilde{\sf B}}
\newcommand{\Dom}{\operatorname{Dom}}
\renewcommand{\Dom}{\operatorname{\mathcal D}}
\newcommand{\Ran}{\operatorname{Ran}}
\newcommand{\ebar}{\underline{e}}
\newcommand{\tbar}{\underline{t}}

%\newcommand{\inch}[1]{{\widetilde{#1}}}  % notation for a vector in $\cH$ regarded as a vector in $\tilcH$
\newcommand{\inch}[1]{{#1}^\sharp}  % notation for a vector in $\cH$ regarded as a vector in $\tilcH$

\newcommand{\onenorm}[1]{\Vert#1\Vert_{L^1(\tau)}}  % NC L^1-norm
\newcommand{\twonorm}[1]{\Vert#1\Vert_{L^2(\mu)}}  % L^2-seminorm for functions on X

\newcommand{\clos}[2][]{\overline{#2}^{#1}}
\newcommand{\WOT}{{\operatorname{WOT}}}
\newcommand{\uweak}[1]{\ensuremath{\sigma(#1,{#1}_*)}}

\newcommand{\cu}[1]{{#1}_{\rm un}} % ad hoc conditional unitization


